A Complete Axiomatisation for Quantifier-Free Separation Logic

We present the first complete axiomatisation for quantifier-free separation logic. The logic is equipped with the standard concrete heaplet semantics and the proof system has no external feature such as nominals/labels. It is not possible to rely completely on proof systems for Boolean BI as the concrete semantics needs to be taken into account. Therefore, we present the first internal Hilbert-style axiomatisation for quantifier-free separation logic. The calculus is divided in three parts: the axiomatisation of core formulae where Boolean combinations of core formulae capture the expressivity of the whole logic, axioms and inference rules to simulate a bottom-up elimination of separating connectives, and finally structural axioms and inference rules from propositional calculus and Boolean BI with the magic wand.

==> definition-symbolic-composition.tex <==
In this section we provide useful information on the symbolic composition $\asymbunion$ evoked in Section~\ref{section:axiom2starelim}.
\ifLongVersionWithAppendix
We refer the reader to this section for the definitions (central in this appendix) of symbolic memory state, abstraction
of a memory state and characteristic formula.
\fi
We denote with $\pi_i$ the projection map, so that
given a symbolic memory state $\triple{\symbterms}{\amap}{\symbrem}$ over $\pair{\asetvar}{\bound}$, the function
$\pi_1 \circ \amap$ goes from $\symbterms$ to $\symbterms$, whereas $\pi_2 \circ \amap$ goes from $\symbterms$ to  $\interval{1}{\bound}$
($\pi_i$ is the projection on the $i$th component).

We want to characterise the relation $\asymbunion \subseteq \sum_{\asetvar,\bound_1,\bound_2}
\symbdomain{\asetvar}{\bound_1}\times\symbdomain{\asetvar}{\bound_2}\times\symbdomain{\asetvar}{\bound_1+\bound_2}$, on symbolic memory states having satisfiable characteristic formulae, such that
\begin{description}
\item[\lemmalab{(+$_{\mathsf{sms}}$-adequacy)}{compositionproperty}] For all $\pair{\astore}{\aheap}$ and all
$\asms_1$ and $\asms_2$,
respectively over $\pair{\asetvar}{\bound_1}$ and $\pair{\asetvar}{\bound_2}$,
$\triple{\asms_1}{\asms_2}{\symbms{\astore}{\aheap}{\asetvar}{\bound_1+\bound_2}} \in \asymbunion$
iff
$\aheap_1 + \aheap_2 = \aheap$,
$\asms_1 = \symbms{\astore}{\aheap_1}{\asetvar}{\bound_1}$ and
$\asms_2 = \symbms{\astore}{\aheap_2}{\asetvar}{\bound_2}$ for some $\aheap_1$ and $\aheap_2$.
\end{description}
We write $\symbunion{\triple{\symbterms_1}{\amap_1}{\symbrem_1}}{\triple{\symbterms_2}{\amap_2}{\symbrem_2}}{\triple{\symbterms}{\amap}{\symbrem}}$ for
$\triple{\triple{\symbterms_1}{\amap_1}{\symbrem_1}}{\triple{\symbterms_2}{\amap_2}{\symbrem_2}}{\triple{\symbterms}{\amap}{\symbrem}} \in \asymbunion$.
By Lemma~\ref{lemma:msmodelsabs}, if $\asymbunion$ satisfies \ref{compositionproperty}, then it correctly behaves with respect 
to the separating conjunction $\separate$, as follows:
\begin{nscenter}
$\symbunion{\triple{\symbterms_1}{\amap_1}{\symbrem_1}}{\triple{\symbterms_2}{\amap_2}{\symbrem_2}}{\triple{\symbterms}{\amap}{\symbrem}}\quad
\text{iff}\quad
\models \charsymbform{\triple{\symbterms}{\amap}{\symbrem}} \implies \charsymbform{\triple{\symbterms_1}{\amap_1}{\symbrem_1}} \separate \charsymbform{\triple{\symbterms_2}{\amap_2}{\symbrem_2}}$
\end{nscenter}
As shown in Section~\ref{section:axiom2starelim}, $\asymbunion$ cannot be functional in its first two components.
Moreover, in Section~\ref{section:axiom2starelim} we described the membership problem $\triple{\triple{\symbterms}{\amap_1}{\symbrem_1}}{\triple{\symbterms}{\amap_2}{\symbrem_2}}{\triple{\symbterms}{\amap}{\symbrem}} \in \asymbunion$ to be roughly equivalent to the problem of finding
two graph homomorphisms from the graphs $\pair{\symbterms_1}{\amap_1}$ and $\pair{\symbterms_2}{\amap_2}$ to $\pair{\symbterms}{\amap}$,
together with the existence of a partition that guarantees that paths that do not belong to the homomorphisms can be generated using the
%% additional
memory cells from the garbage (abstracted by $\symbrem_1$ and $\symbrem_2$) -- see the details below.
Now, we  define this problem and we give an informal explanation to its components.
\cut{
Notice that $\asymbunion$ cannot be functional on its first two components.
Take for example the symbolic memory state $\asms = (\{\avariable,\ameetvar{\avariable}{\avariable}{\avariable}\},\emptyset,1)$ and let us
ask ourselves for which symbolic memory states $\asms$,  it should hold that $\symbunion{\asms}{\asms}{\asms'}$
There are (at least) two possibilities.
\begin{enumerate}
\item As $\asms$ is the abstraction of the memory states $(\astore,\{\alocation_1\pto\alocation_2\})$ and $(\astore,\{\alocation_2\pto\alocation_1)\})$ where $\astore(\avariable) = \alocation_1 \neq \alocation_2$,
the abstraction of $(\astore,\{\alocation_1\pto\alocation_2,\alocation_2\pto\alocation_1\})$ must be a solution for $\asms'$.
More precisely, this abstraction is
$(\asymbterm,\{\asymbterm \pto (\asymbterm,2) \},0)$ where $\asymbterm = \{\avariable,\ameetvar{\avariable}{\avariable}{\avariable}\}$.
\item However, $\asms$ is  also the abstraction of $(\astore,\{\alocation_1\pto\alocation_2\})$ and $(\astore,\{\alocation_3\pto\alocation_4)\})$ such that $\astore(\avariable) \not\in \{\alocation_1,\alocation_3\}$.
Then, the abstraction $\triple{\{\avariable,\ameetvar{\avariable}{\avariable}{\avariable}\}}{\emptyset}{2}$ must also be a solution for $\asms'$.
\end{enumerate}
From the above example, it is clear what is the main challenge in defining
This possibility was depicted in the first case above.
}

Let $\asms_1 = {\triple{\symbterms_1}{\amap_1}{\symbrem_1}}$, $\asms_2 = {\triple{\symbterms_2}{\amap_2}{\symbrem_2}}$ and $\asms = {\triple{\symbterms}{\amap}{\symbrem}}$ be three symbolic memory states
respectively over $\pair{\asetvar}{\bound_1}$, $\pair{\asetvar}{\bound_2}$ and
$\pair{\asetvar}{\bound_1+\bound_2}$
% The characterisation of $\asymbunion$ that we are tring to achieve is reminiscent of the computation of graph homomorphisms, as paths between program variables in the heaps $\aheap_1$ and $\aheap_2$ are preserved in their composition, with additional conditions that model how paths can be introduced.
We have $\symbunion{\asms_1}{\asms_2}{\asms}$ $\equivdef$ \\

{
\small
\noindent $\charsymbform(\asms_1)$, $\charsymbform(\asms_2)$ and $\charsymbform(\asms)$ are satisfiable
and
there are injections $\ainj_1:\symbterms_1 \to \symbterms$ and $\ainj_2:\symbterms_2 \to \symbterms$
satisfying the following 4 conditions:

\begin{enumerate}
\item[\lemmalab{1}{C-functionality}.] for each $\asymbterm \in \domain{\amap}$ then it cannot be that
$\ainj_1^{-1}(\asymbterm) \in \domain{\amap_1}$ and $\ainj_2^{-1}(\asymbterm) \in \domain{\amap_2}$;
\end{enumerate}

\begin{enumerate}
\item[\lemmalab{2}{C-meet-points}.] for all $i \in \{1,2\}$, for each $\asymbterm \in \symbterms_i$,
  \begin{enumerate}[nosep]
  \item for each $\avariable \in \asetvar$, \ $\avariable \in \asymbterm \iff \avariable \in \ainj_i(\asymbterm)$;
  \item for each meet-point term $\ameetvar{\avariable}{\avariablebis}{\avariableter} \in \asymbterm$,
  if $\ameetvar{\avariablebis}{\avariable}{\avariableter} \not\in \asymbterm$ then
  $\ameetvar{\avariable}{\avariablebis}{\avariableter} \in \ainj_i(\asymbterm)$, otherwise
  $\ameetvar{\avariable}{\avariablebis}{\avariableter} \in \ainj_i(\asymbterm)$ or $\ameetvar{\avariablebis}{\avariable}{\avariableter} \in \ainj_i(\asymbterm)$.
  \end{enumerate}
\end{enumerate}

\begin{enumerate}
\item[\lemmalab{3}{C-homomorphism}.] for all $i \in \{1,2\}$, for all $\aterm_1,\aterm_2 \in \atermset{\asetvar}$ and 
for all $\inbound \in \interval{1}{\bound_i}$, if $\amap_i(\equivclass{\aterm_1}{\symbterms_i}) = (\equivclass{\aterm_2}{\symbterms_i},\inbound)$ then
there is $n \in \Nat$ and a set $\{\asymbterm_0,\dots,\asymbterm_{n+1}\} \subseteq \symbterms$ such that
\begin{enumerate}[nosep]
\item $\asymbterm_0 {=} \ainj_i(\equivclass{\aterm_1}{\symbterms_i})$ and $\asymbterm_{n+1} {=} \ainj_i(\equivclass{\aterm_2}{\symbterms_i})$;
\item for each $j \in \interval{1}{n}$, $\asymbterm_j \not\in\range{\ainj_1} \cup \range{\ainj_2}$;
\item for each $j \in \interval{0}{n}$, $(\pi_1 \circ \amap)(\asymbterm_j) = \asymbterm_{j+1}$;
\item if $\inbound < \bound_i$ then $\sum_{j\in\interval{0}{n}} (\pi_2 \circ \amap)(\asymbterm_j) = \inbound$,
else $\sum_{j\in\interval{0}{n}} (\pi_2 \circ \amap)(\asymbterm_j) \geq \bound_i$.
\end{enumerate}
\end{enumerate}

\noindent Let $\symbsources{\asms_1}{\asms_2}{\asms}$, $\symbtargets{\asms_i}{\asms}$ ($i \in \{1,2\}$) and
$\symbinternal{\asms_1}{\asms_2}{\asms}$ be the sets defined below
\begin{itemize}[nosep]
\item $\symbsources{\asms_1}{\asms_2}{\asms}$ $\egdef$
$\{ \asymbterm \in \symbterms \mid$ $\asymbterm {\cap} \asetvar \neq \emptyset$ and for all $\avariable \in \asymbterm {\cap} \asetvar$ and $i {\in} \{1,2\}$,
$\equivclass{\avariable}{\symbterms_i} {\not \in} \domain{\amap_i}\}$.
\item $\symbtargets{\asms_i}{\asms}$ is the set of $\asymbterm \in \symbterms$\ such that $\asymbterm \cap \asetvar \neq \emptyset$ or there are
$\aterm_1,\aterm_2 \in \atermset{\asetvar}$, $\alength_1,\alength_2 \geq 0$ such that
\begin{itemize}[nosep]
\item $(\pi_1\circ\amap_i)(\equivclass{\aterm_1}{\symbterms_i}) = \equivclass{\aterm_2}{\symbterms_i}$;
\item $(\pi_1 \circ \amap)^{\alength_1}(\ainj_i(\equivclass{\aterm_1}{\symbterms_i})) = \asymbterm$ and
$(\pi_1 \circ \amap)^{\alength_2}(\asymbterm) = \ainj_i(\equivclass{\aterm_2}{\symbterms_i})$;
\item for every $\alength < \alength_1+\alength_2$, $(\pi_2 \circ \amap)^{\alength}(\equivclass{\aterm_1}{\symbterms_i}) \neq \ainj_i(\equivclass{\aterm_2}{\symbterms_i})$.
\end{itemize}
\item
$\symbinternal{\asms_1}{\asms_2}{\asms} \egdef \domain{\amap} \setminus
((\cup_{i\in\{1,2\}}\symbtargets{\asms}{\asms_i}) \setminus \symbsources{\asms_1}{\asms_2}{\asms})$.
\end{itemize}

\cut{
\begin{enumerate}
\item[\lemmalab{4}{C-stillgarbage}.] If $\symbrem_1 < \bound_1$ and $\symbrem_2 < \bound_2$ then
$R \egdef \symbrem +
\sum_{\asymbterm \in \symbinternal{\asms_1}{\asms_2}{\asms}} (\pi_2 \circ \amap)(\asymbterm)$ equals $\symbrem_1 + \symbrem_2$,
else $R \geq \symbrem_1 + \symbrem_2$.
\end{enumerate}
}

\begin{enumerate}
\item[\lemmalab{4}{C-wasgarbage}.]
there are two functions $\amapbis_1,\amapbis_2: \symbinternal{\asms_1}{\asms_2}{\asms} \to \interval{1}{\bound_1+\bound_2}$ and $\symbrem_1',\symbrem_2' \in \Nat$ such that
\begin{enumerate}
\item $\symbrem = \symbrem_1' + \symbrem_2'$ and for every $\asymbterm \in \symbinternal{\asms_1}{\asms_2}{\asms}$, $(\pi_2 \circ \amap)(\asymbterm) = \amapbis_1(\asymbterm) + \amapbis_2(\asymbterm)$;
\item for all $i \in \{1,2\}$,
 $\min(\symbrem_i' + \sum_{\asymbterm \in \symbinternal{\asms_1}{\asms_2}{\asms}} \amapbis_i(\asymbterm), \bound_i) = \min(\symbrem_i, \bound_i)$;
\item for every $\asymbterm \in \symbsources{\asms_1}{\asms_2}{\asms} \cap \domain{\amap}$ there is
$\{\asymbterm_0 {=} \asymbterm, \asymbterm_1,\dots,\asymbterm_n\} \subseteq \symbinternal{\asms_1}{\asms_2}{\asms}$ such that
\begin{itemize}
\item for every
$j \in \interval{0}{n-1}$, $(\pi_1 \circ \amap)(\asymbterm_j) = \asymbterm_{j+1}$;
\item $(\pi_1 \circ \amap)(\asymbterm_n) \in \bigcup_{i \in \{1,2\}} \symbtargets{\asms_i}{\asms}$;
\item given $i \in \{1,2\}$, if $(\pi_1 \circ \amap)(\asymbterm_n) \in \symbtargets{\asms_i}{\asms}$ then
$\sum_{j \in \interval{0}{n}} \amapbis_{(3-i)}(\asymbterm_j) \geq 1$ .
\end{itemize}
\end{enumerate}
\end{enumerate}
\cut{
\begin{enumerate}

\item[\lemmalab{5}{C-wasgarbage}.]
there are two functions $\amapbis_1,\amapbis_2: \symbinternal{\asms_1}{\asms_2}{\asms} \to \interval{1}{\bound_1+\bound_2}$ such that
\begin{enumerate}
\item for all $i \in \{1,2\}$, the sum $\sum_{\asymbterm \in \symbinternal{\asms_1}{\asms_2}{\asms}} \amapbis_i(\asymbterm)$ is at most $\symbrem_i$ whenever $\symbrem_i < \bound_i$;
\item for every $\asymbterm \in \symbinternal{\asms_1}{\asms_2}{\asms}$, $(\pi_2 \circ \amap)(\asymbterm) = \amapbis_1(\asymbterm) + \amapbis_2(\asymbterm)$;
\item for every $\asymbterm \in \symbsources{\asms_1}{\asms_2}{\asms} \cap \domain{\amap}$ there is
$\{\asymbterm_0 {=} \asymbterm, \asymbterm_1,\dots,\asymbterm_n\} \subseteq \symbinternal{\asms_1}{\asms_2}{\asms}$ such that
\begin{itemize}
\item for every
$j \in \interval{0}{n-1}$, $(\pi_1 \circ \amap)(\asymbterm_j) = \asymbterm_{j+1}$;
\item $(\pi_1 \circ \amap)(\asymbterm_n) \in \bigcup_{i \in \{1,2\}} \symbtargets{\asms_i}{\asms}$;
\item given $i \in \{1,2\}$, if $(\pi_1 \circ \amap)(\asymbterm_n) \in \symbtargets{\asms_i}{\asms}$ then
$\sum_{j \in \interval{0}{n}} \amapbis_{(3-i)}(\asymbterm_j) \geq 1$ .
\end{itemize}
\end{enumerate}
\end{enumerate}
}
}

\noindent Let us dissect this involved definition.
First of, notice that we only consider symbolic memory states that abstract concrete ones. This follows directly from the fact that we require $\charsymbform(\asms_1)$, $\charsymbform(\asms_2)$ and $\charsymbform(\asms)$ to be satisfiable (first line in the definition).
The main objects in this definition are the two injections $\ainj_1$ and $\ainj_2$.
Given $i \in \{1,2\}$, the injection $\ainj_i$ goes from elements of $\symbterms_i$ to elements of $\symbterms$. Recall that, by definition of symbolic memory states, members of these sets represent equivalence classes between terms.
Informally speaking, the role of $\ainj_1$ and $\ainj_2$ is then to explain how the terms in $\asms_1$ and $\asms_2$ are updated when the two symbolic memory states are combined into $\asms$.
For the remaining part of the section, let us fix three memory states
$\pair{\astore}{\aheap_1}$, $\pair{\astore}{\aheap_2}$ and $\pair{\astore}{\aheap}$, and let us assume $\asms_1 = \symbms{\astore}{\aheap_1}{\asetvar}{\bound_1} = {\triple{\symbterms_1}{\amap_1}{\symbrem_1}}$, $\asms_2 = \symbms{\astore}{\aheap_2}{\asetvar}{\bound_2} = {\triple{\symbterms_2}{\amap_2}{\symbrem_2}}$
and $\asms = \symbms{\astore}{\aheap}{\asetvar}{\bound_1+\bound_2} = {\triple{\symbterms}{\amap}{\symbrem}}$ to be their abstractions.
The key property of $\ainj_1$ and $\ainj_2$ is that, if $\triple{\asms_1}{\asms_2}{\asms} \in \asymbunion$ holds, then
for every equivalence class $\asymbterm \in \symbterms_i$ ($i \in \{1,2\}$),
the location $\alocation$ corresponding in $\pair{\astore}{\aheap_i}$ to the terms in $\asymbterm$ also corresponds
to the terms in $\ainj_i(\asymbterm)$ w.r.t. $\pair{\astore}{\aheap}$.
Essentially then, each pair in $\ainj_i$ (seen as a binary relation) uniquely corresponds to a location.
When this correspondence is understood, most of the conditions on these two injections are easy to follow.
When possible, we explain these conditions with easy ``small-step'' tautologies of \intervalSL (e.g.\ in \ref{C-meet-points}(a)).
\begin{enumerate}
\item Condition~\ref{C-functionality} essentially tells us that $\symbunion{\asms_1}{\asms_2}{\asms}$ cannot hold if the two symbolic memory states only correspond to concrete models that do not have a disjoint heap domain.
For example, let us consider the symbolic memory state $\asms' = (\asymbterm,\{\asymbterm \pto (\asymbterm,2) \},0)$ where $\asymbterm = \{ \avariable, \ameetvar{\avariable}{\avariable}{\avariable}\}$ and $\avariable \in \asetvar$.
Trivially, it cannot be that there is a symbolic memory state $\asms''$ such that $\symbunion{\asms'}{\asms'}{\asms''}$.
Indeed, every concrete memory state $\pair{\astore'}{\aheap'}$ having $\symbms{\astore'}{\aheap'}{\asetvar}{\bound} = \asms'$ must present a cycle involving the location corresponding to $\avariable$.
Hence, it cannot be that both $\pair{\astore}{\aheap_1}$ and $\pair{\astore}{\aheap_2}$ are abstracted by $\asms'$, as it implies that $\domain{\aheap_1} \cap \domain{\aheap_2} \neq \emptyset$ and therefore
$\aheap_1 + \aheap_2$ is not defined (which is required by \ref{compositionproperty}).
Alternatively, this condition can be easily explained with the formula $\lnot(\seesgeq{\aterm}{\aterm_1}{\asetmeetvar_1}{\inbound_1} \separate \seesgeq{\aterm}{\aterm_2}{\asetmeetvar_2}{\inbound_2})$, which is tautological in \intervalSL.
\item Let us now consider the Condition~\ref{C-meet-points}.
 \ref{C-meet-points}(a) essentially tells us that (dis)equivalences between program variables is preserved, and is better explained just by considering the tautology $\avariable = \avariablebis \iff (\avariable = \avariablebis \separate \true)$ (together with the commutativity of $\separate$).
To explain  \ref{C-meet-points}(b), consider $\pair{\astore}{\aheap_1}$ such that for a meet-point term $\ameetvar{\avariable}{\avariablebis}{\avariableter}$,
we have $\semantics{\ameetvar{\avariable}{\avariablebis}{\avariableter}}_{\astore,\aheap_1} = \alocation$.
Moreover, let $\aheap$
\begin{minipage}{0.8\linewidth}
be such that $\aheap_1 \subheap \aheap$.
The condition \ref{C-meet-points}(b) essentially
states the following:
\begin{itemize}[nosep]
  \item
  if $\ameetvar{\avariable}{\avariablebis}{\avariableter}$ is an asymmetric meet-point then the location $\alocation$ corresponds to $\ameetvar{\avariable}{\avariablebis}{\avariableter}$ also in $\pair{\astore}{\aheap}$. Formally,
  if $\pair{\astore}{\aheap_1} \models \ameetvar{\avariable}{\avariablebis}{\avariableter} \neq \ameetvar{\avariablebis}{\avariable}{\avariableter}$ then
  $\semantics{\ameetvar{\avariable}{\avariablebis}{\avariableter}}_{\astore,\aheap} = \semantics{\ameetvar{\avariable}{\avariablebis}{\avariableter}}_{\astore,\aheap_1}$.
  \item if instead $\ameetvar{\avariable}{\avariablebis}{\avariableter}$ is a symmetric meet-point, then the location $\alocation$ corresponds in $\pair{\astore}{\aheap}$ to at least one term between $\ameetvar{\avariable}{\avariablebis}{\avariableter}$ and $\ameetvar{\avariablebis}{\avariable}{\avariableter}$.
  Formally, if $\pair{\astore}{\aheap_1} \models \ameetvar{\avariable}{\avariablebis}{\avariableter} = \ameetvar{\avariablebis}{\avariable}{\avariableter}$ then
  $\semantics{\ameetvar{\avariable}{\avariablebis}{\avariableter}}_{\astore,\aheap} = \semantics{\ameetvar{\avariable}{\avariablebis}{\avariableter}}_{\astore,\aheap_1}$ or
  $\semantics{\ameetvar{\avariable}{\avariablebis}{\avariableter}}_{\astore,\aheap} = \semantics{\ameetvar{\avariablebis}{\avariable}{\avariableter}}_{\astore,\aheap_1}$.
\end{itemize}
The validity of this condition is pretty straightforward. If $\ameetvar{\avariable}{\avariablebis}{\avariableter}$ is an
asymmetric meet-point, it must be that $\alocation$ belongs to a cycle, as depicted on the first figure on the right.
Then, in every extension of this heap, $\alocation$ must still be the first location reachable from $\avariable$ that belongs to~the~cycle.%
\parfillskip=0pt
\end{minipage}%
\begin{minipage}{0.2\linewidth}
  \begin{flushright}
    \begin{minipage}{0.9\linewidth}
    \begin{tikzpicture}
      \coordinate (cir) at (0,0);
      \def\radius{0.45cm}
      %\draw (cir) circle[radius=\radius];

      \draw (cir) ++(90:\radius) node[highlightnode,label={[xshift=-15pt,yshift=-6pt]{$\scriptstyle{\ameetvar{\avariable}{\avariablebis}{\avariableter}}$}}] (k) {};

      \draw (cir) ++(270:\radius) node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariableter}}$}}] (u) {};

      \node[dot,label={[xshift=0pt]$\scriptstyle{\avariable}$}] (m) [above = 0.5cm of k] {};

      \draw (cir) ++(180:\radius) node[highlightnode,label={[xshift=17pt,yshift=-10pt]$\scriptstyle{
      \ameetvar{\avariablebis}{\avariable}{\avariableter}}$}] (ze) {};

      \node[dot,label=below:{$\scriptstyle{\avariablebis}$}] (z) [left=0.6cm of u] {};

      \draw[pto] (m.center) -- (k);
      \draw[pto] (z.center) -- (ze);

      \draw[pto] (u) .. controls +(0:1) and +(0:1) .. (k);
      \draw[pto] (k) .. controls +(180:0.3) and +(90:0.3) .. (ze);
      \draw[pto] (ze) .. controls +(-90:0.3) and +(180:0.3) .. (u);
    \end{tikzpicture}

    \begin{tikzpicture}
      \coordinate (cir) at (0,0);
      \def\radius{0.45cm}
      %\draw (cir) circle[radius=\radius];

      \draw (cir) ++(90:\radius) node[dot] (k) {};

      \draw (cir) ++(270:\radius) node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariableter}}$}}] (u) {};

      \node[dot,label={[xshift=0pt]$\scriptstyle{\avariable}$}] (m) [above = 0.5cm of k] {};

      \draw (cir) ++(180:\radius) node[highlightnode,label={[xshift=32pt,yshift=-10pt]$\scriptstyle{
      \ameetvar{\avariable}{\avariablebis}{\avariableter}} = \ameetvar{\avariablebis}{\avariable}{\avariableter}$}] (ze) {};

      \node[dot,label=below:{$\scriptstyle{\avariablebis}$}] (z) [left=0.6cm of u] {};

      \draw[pto] (m.center) -- (k);
      \draw[pto] (z.center) -- (ze);

      \draw[pto] (k) .. controls +(180:0.3) and +(90:0.3) .. (ze);
      \draw[pto] (ze) .. controls +(-90:0.3) and +(180:0.3) .. (u);
    \end{tikzpicture}
    \end{minipage}
    \end{flushright}
\end{minipage}

\noindent
Hence, by definition of meet-points, $\alocation$ still corresponds to $\ameetvar{\avariable}{\avariablebis}{\avariableter}$.
If instead $\ameetvar{\avariable}{\avariablebis}{\avariableter}$ is a symmetric meet-point (as depicted on the second figure) then there are essentially three possibilities.
First, it could be that $\ameetvar{\avariable}{\avariablebis}{\avariableter}$ is still a symmetric meet-point in $\pair{\astore}{\aheap}$. Then, as shortest paths are preserved when taking extensions of a heap, this meet-point must correspond to $\alocation$.
If instead $\ameetvar{\avariable}{\avariablebis}{\avariableter}$ is no longer a symmetric meet-point, $\alocation$ now belongs to a cycle. There are essentially two distinct ways to introduce such a cycle.
\begin{itemize}
  \item It could be that the cycle is closed on a location in the path from $\astore(\avariable)$ to $\semantics{\ameetvar{\avariable}{\avariablebis}{\avariableter}}_{\astore,\aheap_1}$ (excluded). Essentially, this means moving from the memory state depicted in the second figure to the one depicted in the first one.
  Then, $\alocation$ corresponds to $\ameetvar{\avariablebis}{\avariable}{\avariableter}$.
  \item It could be that the cycle is closed on a location in the path from $\astore(\avariablebis)$ to $\semantics{\ameetvar{\avariable}{\avariablebis}{\avariableter}}_{\astore,\aheap_1}$ (excluded).
  For instance, in the memory state depicted in the second figure, this can be done by adding a path from $\astore(\avariableter)$ to $\astore(\avariablebis)$. This case is symmetrical to the previous one, and $\alocation$ corresponds to $\ameetvar{\avariable}{\avariablebis}{\avariableter}$.
\end{itemize}

\item
For Condition~\ref{C-homomorphism},
let us start by reasoning on the two concrete memory states $\pair{\astore}{\aheap_1}$ and $\pair{\astore}{\aheap_2}$, and suppose that $\aheap_1 + \aheap_2$ is defined as $\aheap$. By looking at $\aheap$, it could be that new paths between program variables are generated. An example of this is depicted in the following figure, where a non-empty path from $\astore(\avariablebis)$ to itself is introduced.

\noindent\hfill%
\begin{tikzpicture}[baseline]

\node[dot,label={[xshift=0pt]$\scriptstyle{\avariable}$}] (x) at (0,0) {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\alocation}}$}}] (l) [right = 0.7cm of x] {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariablebis}}$}}] (y) [right = 0.7cm of l] {};

\draw[pto] (x.center) -- (l);
\draw[pto] (l.center) -- (y);

\end{tikzpicture}
\qquad\heapsum\qquad
\begin{tikzpicture}[baseline]

\node[dot,label={[xshift=0pt]$\scriptstyle{\avariable}$}] (x) at (0,0) {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\alocation}}$}}] (l) [right = 0.7cm of x] {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariablebis}}$}}] (y) [right = 0.7cm of l] {};

\draw[pto] (y) .. controls +(90:0.6) and +(90:0.6) .. (l);
\end{tikzpicture}
\qquad=\qquad
\begin{tikzpicture}[baseline]

\node[dot,label={[xshift=0pt]$\scriptstyle{\avariable}$}] (x) at (0,0) {};
\node[highlightnode,label={[yshift=-15pt]{$\scriptstyle{{\alocation}}$}}] (l) [right = 0.7cm of x] {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariablebis}}$}}] (y) [right = 0.7cm of l] {};

\draw[pto] (x.center) -- (l);
\draw[pto] (l.center) -- (y);

\draw[pto] (y) .. controls +(90:0.6) and +(90:0.6) .. (l);
\end{tikzpicture}
\hfill\,

Because of this, the truth values of $\mathtt{sees}$ predicates change. Indeed, it is clear that the memory state on the left satisfies $\seesgeq{\avariable}{\avariablebis}{\atermset{\{\avariable,\avariablebis\}}}{2}$.
However, this core formula is  not satisfied in the memory state on the right (the disjoint union), as the location $\alocation$ corresponds to the meet-point term $\ameetvar{\avariable}{\avariablebis}{\avariablebis}$. However, this memory state still satisfies
$\seesgeq{\avariable}{\avariablebis}{\emptyset}{2}$.
Then, Condition~\ref{C-homomorphism} essentially states that paths between locations corresponding to terms are preserved when the heap is extended.
With respect to program variables, this condition can therefore be understood from the tautology
$\seesgeq{\avariable}{\avariablebis}{\asetmeetvar}{\inbound} \separate \true \implies \seesgeq{\avariable}{\avariablebis}{\emptyset}{\inbound}$.
\end{enumerate}
As we just saw, Condition~\ref{C-homomorphism} deals with existing paths between terms, and states that they still exist when a heap is extended. The last condition (Condition~\ref{C-wasgarbage}) mainly deals instead with the new paths, created by the union of two heaps.
This condition uses the sets $\symbsources{\asms_1}{\asms_2}{\asms}$, $\symbtargets{\asms_i}{\asms}$ ($i \in \{1,2\}$) and
$\symbinternal{\asms_1}{\asms_2}{\asms}$, whose role is explained below.
\begin{itemize}
\item The set $\symbsources{\asms_1}{\asms_2}{\asms}$ contains the set of equivalence classes of $\symbterms$ having variables from which it is possible to start new paths.
An example of such a variable is given by $\avariablebis$ in the three memory states introduced in order to explain Condition~\ref{C-homomorphism}.
The key property is that, when considering the two leftmost memory states, $\astore(\avariablebis)$ does not reach
(in at least one step) any location corresponding to terms (formally, for every $i \in \{1,2\}$, $\equivclass{\avariablebis}{\symbterms_i} {\not \in} \domain{\amap_i}\}$).
\item The definition of $\symbtargets{\asms_i}{\asms}$ is more involved. Essentially, it contains the set of equivalence classes in $\symbterms$ corresponding to locations where new paths end.
By considering the example in Condition~\ref{C-homomorphism}, these locations are $\astore(\avariable)$, $\astore(\avariablebis)$ or $\alocation$, where this last location is taken into account since it belongs to the path from $\astore(\avariable)$ to $\astore(\avariablebis)$ of the leftmost memory state.
\item Lastly, $\symbinternal{\asms_1}{\asms_2}{\asms}$ is the set of equivalence classes in $\symbterms$ that corresponds to locations inside new paths. In particular, a member $\asymbterm$ of $\symbinternal{\asms_1}{\asms_2}{\asms}$ satisfies two 
properties.
\begin{itemize}
  \item In the concrete memory state abstracted with $\asms$, $\asymbterm$ corresponds to a location $\alocation$ in the shortest path from a location corresponding to some element in $\symbsources{\asms_1}{\asms_2}{\asms}$ to a location corresponding to an element in $\symbtargets{\asms_i}{\asms}$ (this latter element excluded);
  \item In the concrete memory states abstracted with $\asms_1$ and $\asms_2$, $\alocation$ does not belong to any non-empty path between location corresponding to terms.
\end{itemize}
As an example, let us consider the following three memory states:

\noindent\hfill%
\begin{tikzpicture}[baseline]

\node[dot,label={[xshift=0pt,yshift=-15pt]$\scriptstyle{\alocation}$}] (l) at (0,0) {};
\node[dot,label={[yshift=0pt]{$\scriptstyle{{\avariable}}$}}] (x) [above left = 0.7cm of l] {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariablebis}}$}}] (y) [below left = 0.7cm of l] {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariableter}}$}}] (z) [right = 0.7cm of l] {};

\draw[pto] (x.center) -- (l);
\draw[pto] (y.center) -- (l);

\end{tikzpicture}
\qquad\heapsum\qquad
\begin{tikzpicture}[baseline]

\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\alocation}}$}}] (l) at (0,0) {};
\node[dot,label={[yshift=0pt]{$\scriptstyle{{\avariable}}$}}] (x) [above left = 0.7cm of l] {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariablebis}}$}}] (y) [below left = 0.7cm of l] {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariableter}}$}}] (z) [right = 0.7cm of l] {};

\draw[pto] (l.center) -- (z);

\end{tikzpicture}
\qquad=\qquad
\begin{tikzpicture}[baseline]

\node[highlightnode,label={[xshift=0pt,yshift=-15pt]$\scriptstyle{\alocation}$}] (l) at (0,0) {};
\node[dot,label={[yshift=0pt]{$\scriptstyle{{\avariable}}$}}] (x) [above left = 0.7cm of l] {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariablebis}}$}}] (y) [below left = 0.7cm of l] {};
\node[dot,label={[yshift=-15pt]{$\scriptstyle{{\avariableter}}$}}] (z) [right = 0.7cm of l] {};

\draw[pto] (x.center) -- (l);
\draw[pto] (y.center) -- (l);
\draw[pto] (l.center) -- (z);
\end{tikzpicture}
\hfill\,

\noindent Suppose $\asms_1$, $\asms_2$ and $\asms$ to be the abstractions of these three memory states (from the left to the right).
By definition, both $\symbsources{\asms_1}{\asms_2}{\asms}$ and $\symbtargets{\asms_i}{\asms}$ (for $i \in \{1,2\}$) contain the equivalence classes
$\equivclass{\avariable}{\symbterms}$, $\equivclass{\avariablebis}{\symbterms}$ and $\equivclass{\avariableter}{\symbterms}$.
The equivalence class $\equivclass{\ameetvar{\avariable}{\avariablebis}{\avariableter}}{\symbterms}$ is instead in $\symbinternal{\asms_1}{\asms_2}{\asms}$ (together with $\equivclass{\avariable}{\symbterms}$ and $\equivclass{\avariablebis}{\symbterms}$), as the location $\alocation$ that corresponds to it does not belong to any path between terms in the two subheaps abstracted with $\asms_1$ and $\asms_2$, whereas it belongs to the path from $\equivclass{\avariable}{\symbterms}$ to $\equivclass{\avariableter}{\symbterms}$ in the memory state abstracted with $\asms$.
\end{itemize}
We are now ready to explain Condition~\ref{C-wasgarbage}, which mainly deals with quantitative aspects of the \emph{new paths} generated by the union of memory states.
More precisely, supposing that $\pair{\astore}{\aheap_1}$ and $\pair{\astore}{\aheap_2}$ are such that $\aheap_1 + \aheap_2$ is defined, these paths must be created solely from location in $\domain{\aheap_1}$ or $\domain{\aheap_2}$ that (in both memory states) are not inside paths between locations corresponding to program variables.
From the definition of the symbolic memory states $\asms_1 = {\triple{\symbterms_1}{\amap_1}{\symbrem_1}}$ and $\asms_2 = {\triple{\symbterms_2}{\amap_2}{\symbrem_2}}$, these locations are abstracted with the two quantities $\symbrem_1$ and $\symbrem_2$. These two quantities give precise bounds and constraints on the lengths and the types of paths that can occur in $\asms$. Condition~\ref{C-wasgarbage} faithfully reflects these constraints.
\begin{enumerate}[start=4]
\item  Condition~\ref{C-wasgarbage} makes use of two functions $\amapbis_1$ and $\amapbis_2$, and two quantities $\symbrem_1'$ and $\symbrem_2'$. The role of these objects is, roughly speaking, to explain how the quantities $\symbrem_1$ and $\symbrem_2$ are distributed in $\asms$. Let us be more precise.

Given $i \in \{1,2\}$ and an element $\asymbterm$ in $\symbinternal{\asms_1}{\asms_2}{\asms}$,
$\amapbis_i(\asymbterm)$ reflects the number of locations abstracted with $\symbrem_i$ that are in the path from the location corresponding to $\asymbterm$ to the one corresponding to $\pi_1 \circ \amap(\asymbterm)$ (see \ref{C-wasgarbage}(a)).
Similarly, $\symbrem_i'$ reflects the number of locations abstracted with $\symbrem_i$ that are still garbage locations in $\asms$ (i.e. they are abstracted by $\symbrem$).
Condition~\ref{C-wasgarbage} then distinguishes two cases (both treated by \ref{C-wasgarbage}(b)): $\symbrem_i < \bound_i$ and $\symbrem_i = \bound_i$.
\begin{itemize}
\item If $\symbrem_i < \bound_i$ then, by definition of symbolic memory states, it holds that $\pair{\astore}{\aheap_i}$ (which is abstracted by $\asms_i$) contains exactly $\symbrem_i$ memory cells that are not inside paths between locations corresponding to program variables. Hence, exactly this number of locations must be retrieved from $\symbrem$ and the paths generated by terms in $\symbinternal{\asms_1}{\asms_2}{\asms}$.
This is where $\amapbis_i$ and $\symbrem_i$ come into play, as we require $\symbrem_i' {+} \sum_{\asymbterm \in \symbinternal{\asms_1}{\asms_2}{\asms}} \amapbis_i(\asymbterm)$ to be equal~to~$\symbrem_i$.
\item If instead $\symbrem_i = \bound_i$, by definition of symbolic memory states it holds that $\pair{\astore}{\aheap_i}$ contains at least $\symbrem_i$ memory cells that are not inside paths between locations corresponding to program variables.
Hence, we require $\symbrem_i' + \sum_{\asymbterm \in \symbinternal{\asms_1}{\asms_2}{\asms}} \amapbis_i(\asymbterm)$ to be at least $\symbrem_i$.
\end{itemize}
Lastly, let us briefly explain \ref{C-wasgarbage}(c).
Let us consider a non-empty \emph{new} shortest path from a location corresponding to an equivalence class of $\symbsources{\asms_1}{\asms_2}{\asms}$ to a location corresponding to an equivalence class of $\symbtargets{\asms_i}{\asms}$.
Essentially, as it reaches an element in $\symbtargets{\asms_i}{\asms}$, \ref{C-wasgarbage}(c) states that there must be at least one location in this path that belongs to $\domain{\aheap_{3-i}}$ (i.e. the other heap).
Indeed, if this was not the case, the whole path would belong to the heap $\aheap_i$, and hence it is not generated by the union of the two memory states.
\end{enumerate}


==> paragraph-an-example.tex <==
We develop the proof of $\emp \implies (\alloc{\avariable} \magicwand \size = 1)$ as a more complete example with respect to the one shown in the body of the paper.
We use the following theorem and rules, which can be shown admissible in the calculus:
\begin{nscenter}
  \scalebox{0.9}{
  \lemmalab{\textbf{($\magicwand\land$-DistrL)}}{axiom:magicsep}\,
  $
  (\aformula \magicwand \aformulabis) \land (\aformula \magicwand \aformulater) \implies (\aformula \magicwand \aformulabis \land \aformulater)
  $}%
  \hfill
  \scalebox{0.9}{
  \lemmalab{\textbf{($\land\true$IL)}}{axiom:andtrue}\,
  $
  \aformula \implies \true \land \aformula
  $}%
  \hfill
  \scalebox{0.9}{
  \rulelab{\textbf{$\land$-InfL}}{rule:andinf}
  $
  \inference{\aformula \implies \aformulater}{\aformula \land \aformulabis \implies \aformulater \land \aformulabis}
  $}%
\end{nscenter}
Recall that $\size = \inbound$ is a shortcut for $\size \geq \inbound \land \lnot \size \geq \inbound{+}1$.\\
\scalebox{0.9}{
$
\begin{nd}
\have {5} {\true \separate (\alloc{\avariable} \land \size = 1) \implies (\alloc{\avariable} \land \size = 1) \separate \true} \by{\ref{starAx:Commute}}{}
\have {1} {\alloc{\avariable} \land \size = 1 \implies \size \geq 1} \by{\ref{axiom:andelim}}{}
\have {2} {\alloc{\avariable} \land \size = 1 \separate \true \implies \size \geq 1 \separate \true} \by{\ref{rule:starinference} rule}{1}
\have {3} {\size \geq 1 \separate \true \implies \size \geq 1} \by{\ref{starAx:MonoCore} ($\size \geq 1 \egdef \lnot \emp$)}{}
\have {6} {\true \separate (\alloc{\avariable} \land \size = 1) \implies \size \geq 1} \by{\ref{rule:imptr} twice}{5,2,3}
\have {7} {\true \implies (\alloc{\avariable} \land \size = 1 \magicwand \size \geq 1)} \by{\ref{rule:staradj} rule}{6}
\have {12} {\emp \implies (\alloc{\avariable} \land \size = 1 \magicwand \lnot \size \geq 2)} \by{\small{derived in the body of the paper}}{}
\have {14} {(\alloc{\avariable} \land \size = 1 \magicwand \lnot \size \geq 2) \implies\\
 \true \land (\alloc{\avariable} \land \size = 1 \magicwand \lnot \size \geq 2)} \by{\ref{axiom:andtrue}}{}
\have {15} { \true \land (\alloc{\avariable} \land \size = 1 \magicwand \lnot \size \geq 2) \implies\\
\big((\alloc{\avariable} \land \size = 1 \magicwand \size \geq 1) \land\\ (\alloc{\avariable} \land \size = 1 \magicwand \lnot \size \geq 2)\big)} \by{\ref{rule:andinf}}{7}
\have {16} {\big((\alloc{\avariable} \land \size = 1 \magicwand \size \geq 1) \land\\ (\alloc{\avariable} \land \size = 1 \magicwand \lnot \size \geq 2)\big) \implies\\
(\alloc{\avariable} \land \size = 1 \magicwand \size = 1)
} \by{\ref{axiom:magicsep}}{}
\have {17} {(\alloc{\avariable} \land \size = 1 \magicwand \lnot \size \geq 2) \implies\\ (\alloc{\avariable} \land \size = 1 \magicwand \size = 1)} \by{\ref{rule:imptr} twice}{14,15,16}
\have {18} {\emp \implies
(\alloc{\avariable} \land \size = 1 \magicwand \size = 1)
} \by{\ref{rule:imptr}}{12,17}
\end{nd}
$}


==> proof-lemma-soundness.tex <==
\begin{proof}
%% We omit the intermediate axioms, such as \ref{coreAx:AllocSize}, as they are 
%% provable tautologies in $\coresys(\separate,\magicwand)$.
The validity of axioms~\ref{coreAx:EqRef},\ref{coreAx:EqSub},
\ref{coreAx:PointAlloc} and \ref{coreAx:PointInj} is straightforward.
Moreover, the validity of the axioms~\ref{starAx:Commute},~\ref{starAx:Assoc} and~\ref{starAx:Emp}
and the three rules (\ref{rule:starinference},~\ref{rule:staradj} and~\ref{rule:magicwandadj}) is inherited from Boolean BI
(see~\cite{Brotherston&Villard14} and~\cite[Section 2]{Galmiche&Larchey06}).

\begin{itemize}
\item The proof of every instantiation of \ref{starAx:MonoCore} is similar (and quite easy), therefore we show just the case of $\avariable \Ipto \avariablebis \separate \true \implies \avariable \Ipto \avariablebis$.
Suppose $\pair{\astore}{\aheap} \models \avariable \Ipto \avariablebis \separate \true$. Then there is a subheap $\aheap_1 \sqsubseteq \aheap$ such that $\pair{\astore}{\aheap_1} \models \avariable \Ipto \avariablebis$.
Hence, $\aheap_1(\astore(\avariable)) = \astore(\avariablebis)$.
As $\aheap_1 \sqsubseteq \aheap$, we obtain  $\aheap(\astore(\avariable)) = \astore(\avariablebis)$ which by definition implies $\pair{\astore}{\aheap} \models \avariable \Ipto \avariablebis$.
\item \ref{starAx:AllocNeg}.
Suppose $\pair{\astore}{\aheap} \models \lnot \alloc{\avariable} \separate \lnot \alloc{\avariable}$. Then there are
two disjoint heaps $\aheap_1,\aheap_2$ such that $\aheap = \aheap_1 + \aheap_2$, $\pair{\astore}{\aheap_1} \models \lnot \alloc{\avariable}$ and $\pair{\astore}{\aheap_2} \models \lnot \alloc{\avariable}$.
Then $\astore(\avariable) \not \in \domain{\aheap_1}$ and $\astore(\avariable) \not \in \domain{\aheap_2}$.
Since $\aheap = \aheap_1 + \aheap_2$, $\domain{\aheap} = \domain{\aheap_1}\cup\domain{\aheap_2}$ and therefore
$\astore(\avariable) \not \in \domain{\aheap}$.
We conclude that $\pair{\astore}{\aheap} \models \lnot \alloc{\avariable}$.
\item \ref{starAx:PointsNeg}.
Suppose $\pair{\astore}{\aheap} \models (\alloc{\avariable} \land \lnot \avariable \Ipto \avariablebis) \separate \true$.
Then there is a subheap $\aheap_1 \sqsubseteq \aheap$ such that $\pair{\astore}{\aheap_1} \models \alloc{\avariable} \land \lnot \avariable \Ipto \avariablebis$.
Hence, $\astore(\avariable) \in \domain{\aheap_1}$ and $\aheap_1(\astore(\avariable)) \neq \astore(\avariablebis)$.
As $\aheap_1 \sqsubseteq \aheap$, we obtain  $\astore(\avariable) \in \domain{\aheap}$ and $\aheap(\astore(\avariable)) \neq \astore(\avariablebis)$ which by definition implies $\pair{\astore}{\aheap} \models \lnot \avariable \Ipto \avariablebis$.
\item \ref{starAx:AllocSizeOne}. Suppose $\pair{\astore}{\aheap} \models \alloc{\avariable}$.
Then $\astore(\avariable) \in \domain{\aheap}$. Let $\aheap_1 \egdef \{\astore(\avariable)\pto\aheap(\astore(\avariable))\}$. Trivially, $\aheap_1 \sqsubseteq \aheap$ and
$\pair{\astore}{\aheap_1} \models \alloc{\avariable} \land \size = 1$.
We define $\aheap_2$ as the heap such that $\aheap_2 + \aheap_1 = \aheap$.
Trivially, $\pair{\astore}{\aheap_2} \models \true$.
Hence, $\pair{\astore}{\aheap} \models (\alloc{\avariable} \land \size = 1) \separate \true$.

The proof of validity of \ref{starAx:SizeOne} is similar.
\item \ref{starAx:SizeNeg}.
We suppose that $\inbound_1,\inbound_2\geq 1$, as the formula $\lnot \size \geq 0$ is by definition $\lnot \true$ and therefore is unsatisfiable.
Hence, the axiom~\ref{starAx:SizeNeg} is trivially valid by the axiom~\ref{starAx:False} for $\inbound_1$ and $\inbound_2$ equal to $0$.
Suppose $\pair{\astore}{\aheap} \models \lnot \size \geq \inbound_1 \separate \lnot \size \geq \inbound_2$.
Then there are two disjoint heaps $\aheap_1,\aheap_2$ such that $\aheap_1 + \aheap_2 = \aheap$, $\pair{\astore}{\aheap_1} \models \lnot \size \geq \inbound_1$ and $\pair{\astore}{\aheap_2} \models \lnot \size \geq \inbound_2$.
Then, by definition of $\size$, $\card{\domain{\aheap_1}} \leq \inbound_1-1$ and $\card{\domain{\aheap_2}} \leq \inbound_2-1$.
Then, as $\domain{\aheap} = \domain{\aheap_1}\cup\domain{\aheap_2}$, we obtain $\card{\domain{\aheap}} \leq \inbound_1+\inbound_2-2$, which implies
$\pair{\astore}{\aheap} \models \lnot \size \geq \inbound_1+\inbound_2 \dotminus 1$.
\item \ref{starAx:SizeTwo}. Suppose $\pair{\astore}{\aheap} \models \alloc{\avariable} \land \alloc{\avariablebis} \land \avariable \neq \avariablebis$. Then
by definition,
$\astore(\avariable) \neq \astore(\avariablebis)$ and both $\astore(\avariable)$ and $\astore(\avariablebis)$ are in $\domain{\aheap}$. Hence $\card{\domain{\aheap}} \geq 2$, which implies $\pair{\astore}{\aheap} \models \size \geq 2$.
\item \ref{wandAx:Size}. Let $\asetvar\subseteq_\fin\PVAR$ and  $\pair{\astore}{\aheap}$ be a memory state.
Let $\aheap_1$ be a heap of size one such that $\aheap_1(\alocation) = \alocation$ for some $\alocation \not \in \domain{\aheap}\cup\astore(\asetvar)$.
Trivially $\pair{\astore}{\aheap_1}\models \size = 1 \land \bigwedge_{\avariable \in \asetvar} \lnot \alloc{\avariable}$.
Moreover $\aheap_1\perp\aheap$ holds, hence $\aheap_1+\aheap_2$ is defined and $\pair{\astore}{\aheap+\aheap_1} \models \true$.
Then, $\pair{\astore}{\aheap} \models (\size = 1 \land \bigwedge_{\avariable \in \asetvar} \lnot \alloc{\avariable}) \septraction \true$.
\item \ref{wandAx:PointsTo}. Suppose $\pair{\astore}{\aheap} \models \lnot \alloc{\avariable}$.
Let $\aheap_1$ be the heap of size one such that $\aheap_1(\astore(\avariable)) = \astore(\avariablebis)$.
Trivially, $\pair{\astore}{\aheap} \models \avariable \Ipto \avariablebis \land \size = 1$. Moreover, as $\astore(\avariable) \not\in\domain{\aheap}$, $\aheap_1\perp\aheap$ holds, hence $\aheap_1+\aheap_2$ is defined and $\pair{\astore}{\aheap+\aheap_1} \models \true$.
Then, $\pair{\astore}{\aheap} \models (\avariable \Ipto \avariablebis \land \size=1) \septraction \true$.
\item \ref{wandAx:Alloc}. Let $\asetvar \subseteq_\fin \PVAR$ and
suppose $\pair{\astore}{\aheap} \models \lnot \alloc{\avariable}$.
Let $\aheap_1$ be the heap of size one such that $\aheap_1(\astore(\avariable)) = \alocation$ where $\alocation \not \in \astore(\asetvar)$.
Trivially, $\pair{\astore}{\aheap_1} \models \alloc{\avariable} \land \size = 1 \land \bigwedge_{\avariablebis \in \asetvar} \lnot \avariable \Ipto \avariablebis$.
Moreover, as $\astore(\avariable) \not\in\domain{\aheap}$, $\aheap_1\perp\aheap$ holds, hence $\aheap+\aheap_1$ is defined and $\pair{\astore}{\aheap+\aheap_1} \models \true$.
Then, $\pair{\astore}{\aheap} \models (\alloc{\avariable} \land \size = 1 \land \bigwedge_{\avariablebis \in \asetvar} \lnot \avariable \Ipto \avariablebis) \septraction \true$.\qedhere
\end{itemize}
\end{proof}


==> subsection-composition-sms.tex <==
The proof system $\coresys(\separate,\weirdexists)$ for \intervalSL is defined as
$\coresys(\weirdexists)$ augmented by the axioms and the rule from System~\ref{axioms3:Star}.
Its main ingredient is given by the axiom~\ref{starAx2:StarElim} which, following the description in
Section~\ref{subsection:ingredients}, is clearly a big-step axiom. Indeed, as much as we would like to give a set of small-step axioms as we did for \slSW, we argue that producing such an axiomatisation for \intervalSL is
unfeasible.
In the proof system for \slSW, we found out that given two core types $\aformula$ and $\aformulabis$,
%% the formula
$\aformula \separate \aformulabis$ is equivalent to a conjunction of core formulae literals (see the proof
sketch of Lemma~\ref{lemma:starPSLelim}). Similar results hold for the separating implication $\magicwand$
(Lemma~\ref{lemma:magicwandPSLelim}) and the $\weirdexists$ quantifier. This property of being
equivalent to a simple conjunction of core formulae literals facilitates the design of
small-step axioms.
This is not the case for $\separate$ within \intervalSL: given two core types $\aformula$ and $\aformulabis$,
the formula $\aformula \separate \aformulabis$ is equivalent to a non-trivial disjunction of possibly exponentially many conjunctions.
Because of this, small-step axioms are hard to obtain and  some technical developments are needed in order to produce
%% a sound and complete
an adequate
axiom system.
These developments are centered around the notions of symbolic memory states and characteristic formulae.
A \defstyle{symbolic memory state} is an abstraction on the memory state $\pair{\astore}{\aheap}$ that
is guided by the definition of core formulae, essentially highlighting the properties of
$\pair{\astore}{\aheap}$ that are expressible through these formulae, while removing the ones that are not expressible.
Given $\asetvar \subseteq_{\fin} \PVAR$ and $\bound \in \Nat^+$,
a \defstyle{symbolic memory states} $\asms$ over $\pair{\asetvar}{\bound}$ is
defined as a finite structure $\triple{\symbterms}{\amap}{\symbrem}$ such that
\begin{itemize}[nosep]
\item $\symbterms$ is a partition of a subset of $\atermset{\asetvar}$, encoding (dis)equalities. We introduce
the partial function $\equivclass{\ .\ }{\symbterms}: \atermset{\asetvar} \to \symbterms$ such that
given $\aterm \in \atermset{\asetvar}$ returns $\asymbterm \in \symbterms$ and $\aterm \in \asymbterm$, if it exists;
\item $\amap: \symbterms \to \symbterms\times\interval{1}{\bound}$ is a partial function encoding paths between terms and their length;
\item $\symbrem \in \interval{0}{\bound}$, encoding the number of memory cells (up to $\bound$)
not in paths between terms.
\end{itemize}
We denote with $\symbdomain{\asetvar}{\bound}$ the set of these structures.
The \defstyle{abstraction} $\symbms{\astore}{\aheap}{\asetvar}{\bound}$ of a memory state $\pair{\astore}{\aheap}$ is defined as the symbolic memory state $\triple{\symbterms}{\amap}{\symbrem}$ over $\pair{\asetvar}{\bound}$ such that
\begin{itemize}[nosep]
\item $\symbterms \egdef \{ \{ \aterm_1 \in \atermset{\asetvar} \mid \pair{\astore}{\aheap} \models \aterm_1 = \aterm_2 \} \mid \aterm_2 \in \atermset{\asetvar} \}$;
\item {
\addtolength{\jot}{-4pt}
$
\begin{aligned}[t]
\amap(\asymbterm) = (\asymbterm',\inbound) \, \equivdef \,
& \text{there are}\ \aterm_1 {\in} \asymbterm\ \text{and}\
\aterm_2 {\in} \asymbterm'\ \text{such that}\ \pair{\astore}{\aheap} \models \seesgeq{\aterm_1}{\aterm_2}{\atermset{\asetvar}}{\inbound}\ \text{and}\\
&\text{if}\ \inbound < \bound\ \text{then}\
\pair{\astore}{\aheap} \models \lnot \seesgeq{\aterm_1}{\aterm_2}{\atermset{\asetvar}}{\inbound{+}1};
\end{aligned}
$}
\item $\symbrem = \inbound$ $\equivdef$ $\pair{\astore}{\aheap} \models \remgeq{\atermset{\asetvar}\times\atermset{\asetvar}}{\inbound}$ and if $\inbound < \bound$ then
$\pair{\astore}{\aheap} \models \lnot\remgeq{\atermset{\asetvar}\times\atermset{\asetvar}}{\inbound{+}1}$.
\end{itemize}
Thus, a symbolic memory state $\triple{\symbterms}{\amap}{\symbrem}$ over $\pair{\asetvar}{\bound}$ simply stores the truth values for
 equalities, $\mathtt{sees}$ and $\mathtt{rem}$ predicates with respect to a memory state.
Its semantics
is best given through
%%  the following formula of $\conjcomb{\coreformulae{\asetvar}{\bound}}$, denoted with
the \defstyle{characteristic formula} $\charsymbform\triple{\symbterms}{\amap}{\symbrem}$ defined below (sets understood as conjunctions):
\begin{nscenter}
$
\begin{aligned}[t]
&
\formulasubset{\rem{\atermset{\asetvar}\times\atermset{\asetvar}}{\sim}{\symbrem}}{\bmat[\text{if } \symbrem {\neq} \bound \text{ then } (\sim \text{ is } =) \text{ else } (\sim \text{ is } \geq)]}
\land\formulasubset{\aterm_1 \neq \aterm_2}{\bmat[\equivclass{\aterm_1}{\symbterms}\ \text{or}\ \equivclass{\aterm_2}{\symbterms}\ \text{undefined, or}\ \equivclass{\aterm_1}{\symbterms}\neq\equivclass{\aterm_2}{\symbterms}]}
 \\
& {\land}\formulasubset{\aterm_1 = \aterm_2}{\bmat[\equivclass{\aterm_1}{\symbterms}=\equivclass{\aterm_2}{\symbterms} \ \text{defined}]}
  \land
  \formulasubset{\lnot\sees{\aterm_1}{\aterm_2}{\atermset{\asetvar}}}{\bmat[
  \equivclass{\aterm_1}{\symbterms}\ \text{undefined or}\
  \forall\inbound\in\interval{1}{\bound}: \amap(\equivclass{\aterm_1}{\symbterms}) \neq (\equivclass{\aterm_2}{\symbterms},\inbound)]}
  \\
&{\land}
\formulasubset{\sees{\aterm_1}{\aterm_2}{\atermset{\asetvar}}{=}{\inbound}}{\bmat[
\amap(\equivclass{\aterm_1}{\symbterms}) = (\equivclass{\aterm_2}{\symbterms},\inbound)\ \text{and}\ \inbound < \bound]}
\land
\formulasubset{\seesgeq{\aterm_1}{\aterm_2}{\atermset{\asetvar}}{\inbound}}{\bmat[
\amap(\equivclass{\aterm_1}{\symbterms}) = (\equivclass{\aterm_2}{\symbterms},\inbound)\ \text{and}\ \inbound = \bound]}
\end{aligned}
$
\end{nscenter}
From the definitions of $\charsymbform(\asms)$ and $\symbms{\astore}{\aheap}{\asetvar}{\bound}$, we can easily prove the following result.
\begin{restatable}{lemma}{lemmamsmodelsabs}\label{lemma:msmodelsabs}
For every $\pair{\astore}{\aheap}$ and every
$\asms \in \symbdomain{\asetvar}{\bound}$,
$\pair{\astore}{\aheap} \models \charsymbform(\asms)$
%% if and only if
iff $\asms = \symbms{\astore}{\aheap}{\asetvar}{\bound}$.
\end{restatable}%
\noindent Thanks to this lemma, it is easy to see that every satisfiable characteristic formula $\charsymbform(\asms)$ of a symbolic memory state $\asms$ over
$\pair{\asetvar}{\bound}$ is equivalent to exactly one core type in $\coretype{\asetvar}{\bound}$.
Indeed, by definition of core types, the conjunction $\aformula \land \aformulabis$ of two core types $\aformula$ and $\aformulabis$ that are not syntactically equivalent up to associativity and commutativity of $\land$ is unsatisfiable.
Hence, by Lemma~\ref{lemma:msmodelsabs}, if a core type $\aformula \in \coretype{\asetvar}{\bound}$ is satisfied by a memory state $\pair{\astore}{\aheap}$, it must be equivalent to $\charsymbform(\symbms{\astore}{\aheap}{\asetvar}{\bound})$.
By Theorem~\ref{theo:core2PSLcompl} this equivalence is provable in $\coresys$.

The fundamental reason for taking symbolic memory states over memory states is that, given $\asetvar$ and $\bound$, there are finitely many symbolic memory states in $\symbdomain{\asetvar}{\bound}$. This leads to the definition of the
axiom~\ref{starAx2:StarElim}, which given two characteristic formulae $\aformula$ and $\aformulabis$ computes a finite disjunction of characteristic formulae that is equivalent to $\aformula \separate \aformulabis$. This disjunction is defined over a
new composition operator $\asymbunion$ on symbolic memory states that mimicks the
disjoint union $+$ on memory states.
% Then,
% axiom~\ref{starAx2:StarElim}
% is what we need as soon as we can go back and forth between
% the composition of symbolic memory states and the disjoint union of heaps.
More precisely, the following property
shall be satisfied.
\begin{nscenter}
For all $\pair{\astore}{\aheap}$ and all
$\asms_1,\asms_2$ resp. over $\pair{\asetvar}{\bound_1}$ and $\pair{\asetvar}{\bound_2}$,
$\symbunion{\asms_1}{\asms_2}{\symbms{\astore}{\aheap}{\asetvar}{\bound_1+\bound_2}}$
iff there are $\aheap_1$ and $\aheap_2$ such that
$\aheap_1 + \aheap_2 = \aheap$,
$\asms_1 = \symbms{\astore}{\aheap_1}{\asetvar}{\bound_1}$ and
$\asms_2 = \symbms{\astore}{\aheap_2}{\asetvar}{\bound_2}$,
\end{nscenter}
where $\asymbunion \subseteq \sum_{\asetvar,\bound_1,\bound_2} \symbdomain{\asetvar}{\bound_1}\times\symbdomain{\asetvar}{\bound_2}\times\symbdomain{\asetvar}{\bound_1+\bound_2}$,
and $\asms_1$, $\asms_2$  have satisfiable characteristic formulae.
Defining  $\asymbunion$ is clearly challenging.
Unlike the disjoint union of memory states,
$\asymbunion$ is not functional on its first two components. For instance, let
$\asms = (\{\avariable,\ameetvar{\avariable}{\avariable}{\avariable}\},\emptyset,1)$
and let us determine for which  $\asms'$, we have
$\symbunion{\asms}{\asms}{\asms'}$:
\begin{enumerate}[nosep]
\item As $\asms$ is the abstraction of the memory states $(\astore,\{\alocation_1\pto\alocation_2\})$ and $(\astore,\{\alocation_2\pto\alocation_1)\})$ where $\astore(\avariable) = \alocation_1 \neq \alocation_2$,
the abstraction of $(\astore,\{\alocation_1\pto\alocation_2,\alocation_2\pto\alocation_1\})$ must be a solution for $\asms'$.
More precisely, this abstraction is
$(\asymbterm,\{\asymbterm \pto (\asymbterm,2) \},0)$ where $\asymbterm = \{\avariable,\ameetvar{\avariable}{\avariable}{\avariable}\}$.
\item $\asms$ is however also the abstraction of $(\astore,\{\alocation_1\pto\alocation_2\})$ and $(\astore,\{\alocation_3\pto\alocation_4)\})$ such that $\astore(\avariable) \not\in \{\alocation_1,\alocation_3\}$.
Then, the abstraction $\triple{\{\avariable,\ameetvar{\avariable}{\avariable}{\avariable}\}}{\emptyset}{2}$ must also be a solution for $\asms'$.
\end{enumerate}
The main challenge for defining $\asymbunion$ is the composition of the two  ``garbage'':
memory cells that are abstracted with $\symbrem_1$ and $\symbrem_2$ in $\symbms{\astore}{\aheap_1}{\asetvar_1}{\bound_1}$ and $\symbms{\astore}{\aheap_2}{\asetvar_2}{\bound_2}$ may generate new paths between program variables in $\aheap_1+\aheap_2$.
This possibility was depicted in the first case above.
The definition of $\asymbunion$ can be found in
Appendix~\ref{appendix-definition-symbolic-composition}
%% Appendix~\ref{appendix:CompositionMemoryState}
and is too long
to be presented herein.
Roughly speaking,  for $\triple{\triple{\symbterms}{\amap_1}{\symbrem_1}}{\triple{\symbterms}{\amap_2}{\symbrem_2}}{\triple{\symbterms}{\amap}{\symbrem}}$ being in $\asymbunion$,
one needs to witness
two graph homomorphisms from the graphs $\pair{\symbterms_1}{\amap_1}$ and $\pair{\symbterms_2}{\amap_2}$ to $\pair{\symbterms}{\amap}$,
together with the existence of a partition that guarantees that paths that do not belong to the homomorphisms can be generated using the
%% additional
memory cells from the garbage (abstracted by $\symbrem_1$ and $\symbrem_2$).
%%
\LongVersionOnly{
Before introducing the axioms of $\separate$ and complete the axiom system of \intervalSL, it is necessary to do a digression on symbolic memory states.
As we clarified in Section~\ref{subsection:axiom2CoreFormulae}, symbolic memory states link together memory states and core types.
Then, it is natural to ask ourselves how the composition heaps lifts to symbolic memory states.
More explicitly we want to characterise the relation $\asymbunion \subseteq \sum_{\asetvar,\bound_1,\bound_2} \symbdomain{\asetvar_1}{\bound_1}\times\symbdomain{\asetvar_2}{\bound_2}\times\symbdomain{\asetvar}{\bound_1+\bound_2}$ on symbolic memory states having satisfiable characteristic formulae, satisfying the following property:
\begin{description}
\item[] For every $\pair{\astore}{\aheap}$ and every
$\asms_1,\asms_2$ resp. over $\pair{\asetvar}{\bound_1}$ and $\pair{\asetvar}{\bound_2}$,
$\symbunion{\asms_1}{\asms_2}{\symbms{\astore}{\aheap}{\asetvar}{\bound_1+\bound_2}}$
iff there are $\aheap_1$ and $\aheap_2$ such that
$\aheap_1 + \aheap_2 = \aheap$,
$\asms_1 = \symbms{\astore}{\aheap_1}{\asetvar}{\bound_1}$ and
$\asms_2 = \symbms{\astore}{\aheap_2}{\asetvar}{\bound_2}$.
\end{description}
The definition of such a relation is challenging. First of, differently from the union of memory state,
$\asymbunion$ cannot be functional on its first two components. Indeed, let $\asms = (\{\avariable,\ameetvar{\avariable}{\avariable}{\avariable}\},\emptyset,1)$. Lets ask ourselves for which symbolic memory states $\asms'$ it should holds that $\symbunion{\asms}{\asms}{\asms'}$:
\begin{enumerate}
\item As $\asms$ is the abstraction of the memory states $(\astore,\{\alocation_1\pto\alocation_2\})$ and $(\astore,\{\alocation_2\pto\alocation_1)\})$ where $\astore(\avariable) = \alocation_1 \neq \alocation_2$,
the abstraction of $(\astore,\{\alocation_1\pto\alocation_2,\alocation_2\pto\alocation_1\})$ must be a solution for $\asms'$.
More precisely, this abstraction is
$(\asymbterm,\{\asymbterm \pto (\asymbterm,2) \},0)$ where $\asymbterm = \{\avariable,\ameetvar{\avariable}{\avariable}{\avariable}\}$.
\item However, $\asms$ is  also the abstraction of $(\astore,\{\alocation_1\pto\alocation_2\})$ and $(\astore,\{\alocation_3\pto\alocation_4)\})$ such that $\astore(\avariable) \not\in \{\alocation_1,\alocation_3\}$.
Then, the abstraction $\triple{\{\avariable,\ameetvar{\avariable}{\avariable}{\avariable}\}}{\emptyset}{2}$ must also be a solution for $\asms'$.
\end{enumerate}
It is clear what is the main challenge in defining $\asymbunion$: memory cells that are abstracted with $\symbrem_1$ and $\symbrem_2$ in $\symbms{\astore}{\aheap_1}{\asetvar_1}{\bound_1}$ and $\symbms{\astore}{\aheap_2}{\asetvar_2}{\bound_2}$ can generate new paths between program variables in $\aheap_1+\aheap_2$.
This possibility was depicted in the first case above.
\emph{The definition of $\asymbunion$ can be found in Appendix~\ref{appendix:CompositionMemoryState}}.
Informally, solving the inclusion problem of a triple of symbolic memory states $\triple{\triple{\symbterms_1}{\amap_1}{\symbrem_1}}{\triple{\symbterms_2}{\amap_2}{\symbrem_2}}{\triple{\symbterms}{\amap}{\symbrem}}$ in $\asymbunion$ can be reduced to the computation of
two graph homomorphisms from the graphs $\pair{\symbterms_1}{\amap_1}$ and $\pair{\symbterms_2}{\amap_2}$ to $\pair{\symbterms}{\amap}$, together with the computation of a partition problem that checks if paths that do not belongs to the homomorphisms can be generated using the additional memory cells represented with the quantities $\symbrem_1$ and $\symbrem_2$.
The definition of $\asymbunion$ lead us to a concise set of axioms (System~\ref{axioms3:Star}) that allows us to handle the $\separate$ conjunction and therefore obtain an axiomatisation of \intervalSL.
}

